Precise, super-resolving intensity measurement by quantum jump spectroscopy of a single neutral atom

We present precise, sub-wavelength optical intensity measurement using a single trapped $^{87}$Rb atom as a sensor. The intensity is measured by the scalar ac Stark shift it produces on the $F=1 \rightarrow F'=2$ hyperfine transition of the D$_{2}$ line, chosen for its $F' = F+1$ structure and very small tensor polarizability. To boost signal and reduce measurement-induced perturbations, we use a quantum jump spectroscopy technique in which a single absorbed photon on a transition of interest induces the scattering of hundreds of photons on a bright closed transition. The method greatly reduces systematic effects associated with the atomic state, optical polarization, probe power, and atom heating, and gives the atomic temperature as a second spectroscopic observable. We demonstrate the method by measuring the intensity at the focus of an optical tweezer.

==> NewCommands.tex <==
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\sinc}{\mbox{\rm sinc}}
\newcommand{\ba}{{\bf a}}
\newcommand{\bb}{{\bf b}}
\newcommand{\bd}{{\bf d}}
\newcommand{\bk}{{\bf k}}
\newcommand{\bq}{{\bf q}}
\newcommand{\bJ}{{\bf J}}
\newcommand{\bj}{{\bf j}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bx}{{\bf x}}
%\newcommand{\br}{{\bf r}}
\newcommand{\bH}{{\bf H}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bP}{{\bf P}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bv}{{\bf v}}
\newcommand{\brho}{{\bf \rho}}
% \newcommand{\bB}{{\bf B}}
% \newcommand{\bB}{{\bf B}}
% \newcommand{\bB}{{\bf B}}
\newcommand{\balpha}{\stackrel{\leftrightarrow}{\alpha}}
\newcommand{\twovector}[2]{\left[\begin{array}{c}#1\\#2\end{array}\right]}
\newcommand{\twomatrix}[4]{\left[\begin{array}{cc}#1&#2\\#3&#4\end{array}\right]}
\newcommand{\threevector}[3]{\left[\begin{array}{c}#1\\#2\\#3\end{array}\right]}
\newcommand{\threematrix}[9]{
\left[\begin{array}{ccc}#1&#2&#3\\#4&#5&#6\\#7&#8&#9\end{array}\right]}
\newcommand{\braket}[2]{\left<#1|#2\right>}
\newcommand{\ket}[1]{\left|#1\right>}
\newcommand{\bra}[1]{\left<#1\right|}
\newcommand{\Schrodinger}{Schr\"{o}dinger~}
\newcommand{\FigWidth}{15 cm}
\newcommand{\expect}[1]{\left<#1\right>}
\newcommand{\adag}{{a^\dagger}}
%\newcommand{\Tr}{{\rm Tr}}
\newcommand{\chione}{\chi^{(1)}}
\newcommand{\chitwo}{\chi^{(2)}}
\newcommand{\chithr}{\chi^{(3)}}
\newcommand{\deff}{d_{\rm eff}}
\newcommand{\bee}{{\bf e}}
\newcommand{\bA}{{\bf A}}
\newcommand{\bnab}{{\bf \nabla}}
\newcommand{\epzero}{\varepsilon_{0}}
% \newcommand{\bB}{{\boldmath B}}
% \newcommand{\bH}{{\boldmath H}}
\newcommand{\exercise}{\hspace{-.25in}\Large}
\newcommand{\hH}{\hat H}
\newcommand{\hn}{\hat n}
\newcommand{\ha}{\hat a}
\newcommand{\hd}{\hat d}
\newcommand{\hx}{\hat x}
\newcommand{\hp}{\hat p}
\newcommand{\hadagger}{\hat a^{\dagger}}
\newcommand{\hb}{\hat b}
\newcommand{\hbdag}{\hat b^{\dagger}}
\newcommand{\hau}{\hat{\underline{a}}}
\newcommand{\haudagger}{\hau^{\dagger}}
\newcommand{\hbA}{\hat b_{A}}
\newcommand{\hbE}{\hat b_{E}}
\newcommand{\hE}{\hat {\bf E}}
\newcommand{\hnbE}{\hat {E}}
\newcommand{\hnbD}{\hat {D}}
\newcommand{\hEp}{\hat {E}^{(+)}}
\newcommand{\hEm}{\hat {E}^{(-)}}
\newcommand{\hX}{\hat {X}}
\newcommand{\tbE}{{\bf\cal E}}
\newcommand{\tbF}{{\bf\cal F}}
\newcommand{\Ep}{E^{(+)}}
\newcommand{\Em}{E^{(-)}}
\newcommand{\tbX}{{\bf\cal X}}
\newcommand{\tP}{{\cal P}}
\newcommand{\tbP}{{\bf\cal P}}
\newcommand{\tE}{{\cal E}}
\newcommand{\tF}{{\cal F}}
\newcommand{\tG}{{\cal G}}
\newcommand{\tX}{{\cal X}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cP}{{\cal P}}
\newcommand{\nn}{\nonumber \\ }
\newcommand{\nnn}{\nonumber \\ &  &}
\newcommand{\nne}{\nonumber \\ & = &}
\newcommand{\nnequiv}{\nonumber \\ & \equiv &}
\newcommand{\nnapprox}{\nonumber \\ & \approx &}
\newcommand{\nnpropto}{\nonumber \\ & \propto &}
\newcommand{\nnp}{\nonumber \\ & & +}
\newcommand{\nnm}{\nonumber \\ & & -}
\newcommand{\nnt}{\nonumber \\ & & \times}
\newcommand{\bdp}{\bd^{(+)}}
\newcommand{\bdm}{\bd^{(-)}}
\newcommand{\bEp}{\bE^{(+)}}
\newcommand{\bEm}{\bE^{(-)}}
\newcommand{\bBp}{\bB^{(+)}}
\newcommand{\bBm}{\bB^{(-)}}
\newcommand{\hain}{\ha_{\rm IN}}
\newcommand{\haout}{\ha_{\rm OUT}}
\newcommand{\hadaggerin}{\hadagger_{\rm IN}}
\newcommand{\hadaggerout}{\hadagger_{\rm OUT}}
\newcommand{\hEin}{\hnbE_{\rm IN}}
\newcommand{\hEout}{\hnbE_{\rm OUT}}
\newcommand{\haone}{\ha_1}
\newcommand{\hadaggerone}{\hadagger_1}
\newcommand{\hatwo}{\ha_2}
\newcommand{\hadaggertwo}{\hadagger_2}
\newcommand{\hainone}{\ha_{{\rm IN},1}}
\newcommand{\hadaggerinone}{\hadagger_{{\rm IN},1}}
\newcommand{\haintwo}{\ha_{{\rm IN},2}}
\newcommand{\hadaggerintwo}{\hadagger_{{\rm IN},2}}
\newcommand{\curl}{\nabla \times}
\newcommand{\ve}{\varepsilon}
\newcommand{\Adagger}{A^{\dagger}}
\newcommand{\Bdagger}{B^{\dagger}}
\newcommand{\Cdagger}{C^{\dagger}}
\newcommand{\Ddagger}{D^{\dagger}}
\newcommand{\Lag}{{\cal L}}
\newcommand{\var}{{\rm var}}
%\newcommand{\cov}{{\rm cov}}

\newcommand{\PRLsection}[1]{\noindent {\it#1} -}


\newcommand{\arctanh}{\rm{arctanh}}

%\newcommand{\Pe}{P^{\ket{e}}}
%\newcommand{\Pg}{P^{\ket{g}}}
\newcommand{\Pe}{P_e}
\newcommand{\Pg}{P_g}
\newcommand{\PeZ}{P_{e0}}
\newcommand{\PgZ}{P_{g0}}




\newcommand{\supi}{^{(i)}}
\newcommand{\supj}{^{(j)}}
\newcommand{\supij}{^{(i,j)}}


%\newcommand{\mcite}[1]{\cite{#1}}
%\newcommand{\pcite}[1]{\cite{#1}.}
%\newcommand{\ccite}[1]{\cite{#1},}
%
%\newcommand{\mciteSI}[1]{~\citeSI{#1}}
%\newcommand{\pciteSI}[1]{~\citeSI{#1}.}
%\newcommand{\cciteSI}[1]{~\citeSI{#1},}


\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\sigplus}{\sigma ^ +}
\newcommand{\sigmin}{\sigma^-}
\newcommand{\mean}[1]{\langle #1 \rangle}
\renewcommand{\S}{\hat{S}}
\newcommand{\F}{\hat{ F}}
%\newcommand{\var}[1]{\mathrm{var} \left(  #1 \right) }
\renewcommand{\var}{\mathrm{var} }
\newcommand{\Emag}{E_{\mathrm{mag}}}
 \newcommand{\Tone}{\ensuremath{\mathcal{T}_1} }
\newcommand{\Ttwo}{\ensuremath{\mathcal{T}_2} }
\newcommand{\rb}{\ensuremath{ ^{87}\mathrm{Rb} } }
\newcommand{\spinor}[1]{\left( #1 \right)^T }
\newcommand{\Ttot}{T_{\rm acq}}
%\newcommand{\NA}{N_{\rm A}}
\newcommand{\NL}{N_{\rm P}}
%\newcommand{\bF}{\vec{F}}
\newcommand{\bS}{\vec{S}}


\newcommand{\br}{{\bf r}}
%\newcommand{\bk}{{\bf k}}
\newcommand{\bff}{{\bf f}}
\newcommand{\MeasDur}{T_{m}}
